Uncertainty quantification for ptychography using normalizing flows

Ptychography, as an essential tool for high-resolution and nondestructive material characterization, presents a challenging large-scale nonlinear and non-convex inverse problem; however, its intrinsic photon statistics create clear opportunities for statistical-based deep learning approaches to tackle these challenges, which has been underexplored. In this work, we explore normalizing flows to obtain a surrogate for the high-dimensional posterior, which also enables the characterization of the uncertainty associated with the reconstruction: an extremely desirable capability when judging the reconstruction quality in the absence of ground truth, spotting spurious artifacts and guiding future experiments using the returned uncertainty patterns. We demonstrate the performance of the proposed method on a synthetic sample with added noise and in various physical experimental settings.

==> macros2.tex <==
% SIAM Shared Information Template
% This is information that is shared between the main document and any
% supplement. If no supplement is required, then this information can
% be included directly in the main document.


% Packages and macros go here
% \usepackage{lipsum}
 \usepackage{amsfonts}
\usepackage{graphicx}
\usepackage{epstopdf}
\usepackage{mathrsfs}
% \usepackage{algorithmic}
% \usepackage{geometry}
% \geometry{verbose,letterpaper}
% \usepackage{movie15}
\usepackage{hyperref}
%\usepackage{algorithm,algorithmic} % Commented out since loaded previously
%\usepackage{graphicx}
\usepackage{amsmath}
\usepackage{amsfonts}
% \usepackage{amsthm}
% \usepackage{fullpage}
% \usepackage{amssymb}
\usepackage{latexsym}
% \usepackage{pstricks}
% \usepackage{setspace}
%\usepackage{subfig}
\usepackage{comment}
\usepackage{color}
\usepackage{listings}
\usepackage{placeins}
% \usepackage{float}
%\usepackage{tikz,pgflibraryplotmarks}
% \usepackage[percent]{overpic}
\usepackage{subcaption}
\usepackage[labelfont=bf]{caption}
\usepackage{cleveref}
\usepackage{bm}
%\renewcommand{\bf}{\bm}
% \usepackage[font=footnotesize]{caption}
% \usepackage{wrapfig}
% \usepackage{booktabs}
%\usepackage{multirow}
%\ifpdf
%  \DeclareGraphicsExtensions{.eps,.pdf,.png,.jpg}
%\else
%  \DeclareGraphicsExtensions{.eps}
%\fi

% Prevent itemized lists from running into the left margin inside theorems and proofs
\usepackage{enumitem}
\setlist[enumerate]{leftmargin=.5in}
\setlist[itemize]{leftmargin=0.25in}

% Add a serial/Oxford comma by default.
\newcommand{\creflastconjunction}{, and~}
\newcommand{\ie}{i.e.,}

% Used for creating new theorem and remark environments

% Sets running headers as well as PDF title and authors



\usepackage{amsopn}
% \DeclareMathOperator{\diag}{diag}
\graphicspath{{figures/}}

\newcommand {\R}   {{\rm I\!R}}
\newcommand {\uu}  { {\bf u} }
\newcommand {\xx}  { {\bf x} }
\newcommand {\yy}  { {\bf y} }
\newcommand {\hh}  { {\bf h} }
\newcommand {\rr}  { {\bf r} }
\newcommand {\EE}  { {\bf E} }
\newcommand {\HH}  { {\bf H} }
\newcommand {\JJ}  { {\bf J} }
\newcommand {\veps} {\varepsilon}
\newcommand {\Ro} { {\cal R}}
\newcommand {\lag} { {\cal L}}
\newcommand {\sci} { {\rm i}}
\newcommand {\qq}  { {\bf q} }
\newcommand {\pp}  { {\bf p} }
\newcommand {\mm}  { {\bf m} }
\newcommand {\vv}  { {\bf v} }
\newcommand {\ff}  { {\bf f} }
\newcommand {\bb}  { {\bf b} }
\newcommand {\cc}  { {\bf c} }
\newcommand {\dd}  { {\bf d} }
\newcommand {\blambda}  { {\boldsymbol \lambda} }
\newcommand {\bmu}  { {\boldsymbol \mu} }
\newcommand {\bfxi}  { {\boldsymbol \xi} }

\newcommand {\zero}  { {\bf 0} }
\newcommand {\gb}  { {\bf g} }
\newcommand {\bnabla} { { \boldsymbol \nabla} }
\newcommand {\btheta} { { \boldsymbol \theta} }
\newcommand {\balpha} { { \boldsymbol \alpha} }
\newcommand {\bxi} { { \boldsymbol \xi} }
\newcommand {\fuu}  { {\frac{\partial (f_u^T\lambda)}{\partial u}} }
\newcommand {\fum}  { {\frac{\partial (f_u^T\lambda)}{\partial m}} }
\newcommand {\fmm}  { {\frac{\partial (f_m^T\lambda)}{\partial m}} }
\newcommand {\sg}{{\sigma}}
\newcommand{\hf}{\frac12}
\newcommand{\hx}[1]{{\ensuremath{h^x_{\scriptscriptstyle #1}}}}
\newcommand{\hy}[1]{{\ensuremath{h^y_{\scriptscriptstyle #1}}}}
\newcommand{\hz}[1]{{\ensuremath{h^z_{\scriptscriptstyle #1}}}}

\newcommand{\E}{\vec{E}}
\newcommand{\A}{\vec{A}}
\renewcommand{\H}{\vec{H}}
\newcommand{\J}{\vec{J}}
\newcommand{\F}{\vec{F}}
\newcommand{\s}{\vec{s}}
\renewcommand{\u}{\vec{u}}
\newcommand{\B}{{\vec{B}}}
\newcommand{\W}{{\vec{W}}}
\newcommand{\ds}{\displaystyle}
\newcommand{\Fcurly}{\mathcal{F}}
\newcommand{\Dcurly}{\mathcal{D}}
\newcommand{\Ccurly}{\mathcal{C}}
\newcommand{\Rcurly}{\mathcal{R}}
\newcommand{\Dfrakk}{\mathfrak{D}}


\newcommand{\vmu}{\vect{\mu}}
\newcommand{\vx}{\vect{x}}



\newcommand{\calS}{{\cal S}}
\newcommand{\Shj}{{\cal S}_{h}^{j}}


\newcommand{\bfv}{ {\bf{v}}}

\newcommand{\sig}{\sigma}
\newcommand{\hsig}{\widehat \sigma}
\newcommand{\hJ}{\widehat{\vec{J}}}
\newcommand{\nn}{\vec{n}}
% \renewcommand{\div}{\nabla\cdot\,}
\newcommand{\curl}{\ensuremath{{\vec \nabla}\times\,}}
\newcommand{\bbE}{\mathbb{E}}
\newcommand{\bbR}{\mathbb{R}}
\newcommand{\bbC}{\mathbb{C}}
\newcommand{\rme}{\rm{e}}
\newcommand{\mr}{m_{\rm{ref}}}
\newcommand{\wm}{{\widehat m}}
\newcommand{\wy}{{\widehat y}}
\newcommand{\wq}{{\widehat q}}
\newcommand{\wA}{{\widehat A}}
\newcommand{\wB}{{\widehat B}}
\newcommand{\ww}{{\widehat w}}
\newcommand{\bfK}{{\bf K}}

%\newcommand{\diag}{{\sf diag}\, }
\newcommand{\trace}{{\sf trace}\, }
\newcommand*\sepline{%
  \begin{center}
    \rule[1ex]{1.0\textwidth}{.5pt}
  \end{center}}
\newcommand{\TODO}[1]{\textcolor{red}{{\sc Todo:} #1}}

\newcommand{\bfM}{{\bm M}}
\newcommand{\bfC}{{\bm C}}
\renewcommand{\bfK}{{\bm K}}
\newcommand{\bfA}{{\bm A}}
\newcommand{\bfD}{{\bm D}}
\newcommand{\bfE}{{\bm E}}
\newcommand{\bfB}{{\bm B}}
\newcommand{\bfP}{{\bm P}}
\newcommand{\sha}{{\bm G}}
\newcommand{\bfR}{{\bm R}}
\newcommand{\bfJ}{{\bm J}}
\newcommand{\bfL}{{\bm L}}
\newcommand{\bfS}{{\bm S}}
\newcommand{\bfV}{{\bm V}}
\newcommand{\bfI}{{\bm I}}
\newcommand{\bfU}{{\bm U}}
\newcommand{\bfQ}{{\bm Q}}
\newcommand{\bfW}{{\bm W}}
\newcommand{\bfH}{{\bm H}}
\newcommand{\bfF}{{\bm F}}
\newcommand{\bfY}{{\bm Y}}
\newcommand{\bfX}{{\bm X}}
\newcommand{\bfZ}{{\bm Z}}


\newcommand{\bfc}{{\bm c}}
\newcommand{\bfd}{{\bm d}}
\newcommand{\bfe}{{\bm e}}
\newcommand{\bfh}{{\bm h}}
\newcommand{\bfs}{{\bm s}}
\newcommand{\bfm}{{\bm m}}
\newcommand{\bfr}{{\bm r}}
\newcommand{\bfb}{{\bm b}}
\newcommand{\bfa}{{\bm a}}
\newcommand{\bfw}{{\bm w}}
\newcommand{\bff}{{\bm f}}
\newcommand{\bfq}{{\bm q}}
\newcommand{\bfy}{{\bm  y}}
\newcommand{\bfx}{{\bm  x}}
\newcommand{\bfg}{{\bm g}}
\newcommand{\bfu}{{\bm u}}
\newcommand{\bfz}{{\bm z}}
\newcommand{\bft}{{\bm t}}
\newcommand{\bfn}{{\bm n}}
\newcommand{\bfp}{{\bm p}}



\newcommand{\Acurly}{\mathcal{A}}
\newcommand{\Lcurly}{\mathcal{L}}
\newcommand{\Mcurly}{\mathcal{M}}
\renewcommand{\Re}[1]{\operatorname{Re}\left(#1\right)}
\renewcommand{\Im}[1]{\operatorname{Im}\left(#1\right)}

\newcommand{\opt}{\mbox{OPT}}
\newcommand{\bfphi}{{\boldsymbol \Phi}}



\newcommand{\CURL}{{\sf CURL }}
% \newcommand{\DIV}{{\sf DIV }}
\newcommand{\GRAD}{{\sf GRAD }}


\newcommand{\bfepsilon}{\boldsymbol \epsilon}

\newcommand{\yyb}{\bar {\bf y}}
\newcommand{\hhb}{\bar {\bf h}}

\DeclareMathOperator*{\argmin}{arg\,min}                   % arg min
\newtheorem{thm}{Theorem}
\newtheorem{cor}[thm]{Corollary}
\newtheorem{lem}[thm]{Lemma}
\newtheorem{example}{Example}
% \newtheorem{definition}{Definition}


\newcommand{\mat}[1]{\mbox{\boldmath{$#1$}}}
\newcommand{\vect}[1]{\mbox{\boldmath{$#1$}}}
\newcommand{\tens}[1]{\mbox{\boldmath{$#1$}}}
\newcommand{\vecte}[1]{\mbox{\boldmath{$\scriptstyle#1$}}}
\newcommand{\tense}[1]{\mbox{\boldmath{$\scriptstyle#1$}}}
\newcommand{\diag}[1]{\mathrm{diag}\left(#1\right)}
\newcommand{\diff}{\mathrm{d}}
%\newcommand{\dd}[3][]{\frac{\partial^{#1} #2}{\partial #3^{#1}}}
%\newcommand{\ddd}[3][]{\partial^{#1} #2 / \partial #3^{#1}}
%\newcommand{\dn}[1]{\partial_n #1}
\newcommand{\dt}[1]{\partial_t #1}
\newcommand{\e}[1]{\mathrm{\,e}^{#1}}
\newcommand{\x}[1]{\mathrm{\,x}^{#1}}

\DeclareMathOperator{\grad}{{\boldsymbol \nabla}}
\DeclareMathOperator{\grd}{{\boldsymbol \nabla}}
\DeclareMathOperator{\rot}{\boldsymbol \nabla \times}
\DeclareMathOperator{\crl}{\boldsymbol \nabla \times }
\DeclareMathOperator{\dv}{{\boldsymbol \nabla \cdot }}
\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\trot}{\tilde{\boldsymbol \nabla \times}}
\DeclareMathOperator{\tdv}{\tilde{\boldsymbol \nabla \cdot}}
\DeclareMathOperator{\hcrl}{\hat{\boldsymbol \nabla \times}}
\DeclareMathOperator{\hdv}{\hat{\boldsymbol \nabla \cdot}}
\DeclareMathOperator{\vcrl}{\mathbf{\nabla \times}}
\newcommand{\ngrd}[1]{\nabla{#1}}
\newcommand{\nrot}[1]{\nabla\times{#1}}
\newcommand{\ncrl}[1]{\nabla\times{#1}}
\newcommand{\ndv}[1]{\nabla\cdot{#1}}
\newcommand{\nlp}[1]{\nabla^2{#1}}
\DeclareMathOperator{\rank}{rank}
\DeclareMathOperator{\spn}{span}
\newcommand{\mtit}[1]{\text{\itshape #1}} % math text super/subscript
\newcommand{\ibc}[2][\Gamma_{e,j}]{\mathcal{I}_{#1} #2}
\usepackage{mathtools}
\usepackage{url}

\usepackage{mathtools}
\DeclarePairedDelimiter\ceil{\lceil}{\rceil}
\DeclarePairedDelimiter\floor{\lfloor}{\rfloor}

% \newcommand{\mref}{\bfm_\mtit{\rm ref}}
\newcommand{\dm}[1]{\nabla_{\vecte{m}}{#1}}
\newcommand{\dmi}[1]{\nabla_{\vecte{m}_i}{#1}}
\newcommand{\bfSigma}{{\boldsymbol \Sigma}}
\newcommand{\bflambda}{{\boldsymbol \lambda}}

% \usepackage{paralist}
\usepackage{array}
% \usepackage{placeins}

\renewcommand{\figurename}{Fig.}

\newlength{\myrowheight}
\setlength{\myrowheight}{\baselineskip}

% \setlength{\abovedisplayskip}{0pt}
% \setlength{\belowdisplayskip}{0pt}
% \setlength{\abovedisplayshortskip}{0pt}
% \setlength{\belowdisplayshortskip}{0pt}


%%% Local Variables: 
%%% mode:latex
%%% TeX-master: "ex_article"
%%% End: 
\newtheorem{alg}{Algorithm}[section]
\newtheorem{pro}{Proposition}[section]
\newtheorem{defn}{Definition}[section]
\newtheorem{asp}{Assumption}[section]
\newtheorem{rmk}{Remark}[section]
\newtheorem{exmp}{Example}[section]

\newcommand{\WDNote}[1]           % For Wendy's margin notes
{\textcolor{red}{#1}\marginpar{\textcolor{red}{WD $\longleftarrow$}}}



%%%% Custom notes
\newcommand{\wendy}[1]{{{\color{red}{Wendy:} #1}}}
\newcommand{\agni}[1]{\textcolor{blue}{(Agni : #1)}}


%%%% Custom colored text
\newcommand{\blue}[1]{\textcolor{blue}{#1}}
\newcommand{\red}[1]{\textcolor{red}{#1}}
\newcommand{\green}[1]{\textcolor{green}{#1}}


%\newcommand{\carlo}[1]{\textcolor{cyan}{Carlo: #1}}
\newcommand{\citesomething}{\textcolor{red}{Citation Needed}}
